Efficient Inference in Multi-task Cox Process Models

We generalize the log Gaussian Cox process (LGCP) framework to model multiple correlated point data jointly. The observations are treated as realizations of multiple LGCPs, whose log intensities are given by linear combinations of latent functions drawn from Gaussian process priors. The combination coefficients are also drawn from Gaussian processes and can incorporate additional dependencies. We derive closed-form expressions for the moments of the intensity functions and develop an efficient variational inference algorithm that is orders of magnitude faster than competing deterministic and stochastic approximations of multivariate LGCP, coregionalization models, and multi-task permanental processes. Our approach outperforms these benchmarks in multiple problems, offering the current state of the art in modeling multivariate point processes.

==> algorithm.tex <==
	\begin{minipage}{0.49\textwidth}
		\begin{algorithm}[H]
			\caption{LGCPN}\label{LGCPN_code}
			\begin{algorithmic}[1]
				\Inputs{} Observational dataset $\mathcal{D}$, number of latent \gptext{s} $Q$.
				\Output{} Optimized hyper-parameters, posterior moments of $\vecS{\lambda}$
				\Initialize{}  $i \gets 0$, $\allparameters^{(0)} = (\hyperparam, \hyperparam_w, \likeparamvector, \varparam_u, \varparam_w)$,  $\priormeanw \gets 0$, $\priormeanu \gets 0$
				\Repeat
				\State $\max_{\pmb{\mu}} \elbo(\allparameters^{(i)})$
				\State $\allparameters^{(i)} \gets \allparameters^{(i-1)}- \rho \nabla_{\allparameters} \elbo(\allparameters^{(i-1)})$
				\State $i = i +1$
				\Until{convergence criterion is met.}
				\prediction{} $\allparameters^* \gets \allparameters^{(i - 1)}$
				\prediction{} $\mathbb{E}\left[\vecS{\lambda}(\x)^t\right] = \text{exp}(t\likeparamvector^*) \mgf_{\W\f|\allparameters^*}(t)$
			\end{algorithmic}
		\end{algorithm}
	\end{minipage}



==> crime_fig_1.tex <==
% Plot data for crime
\begin{figure}[h]
	\begin{center}
		\includegraphics[width=1\textwidth]{figs/real/crime_data/data_crimegist_heat_r}
		\caption{Counts of crime events on a regular grid. \label{fig:Crime_data}}
	\end{center}
\end{figure}

==> lgcp.tex <==
% Gps and LGCPs

\section{Log-Gaussian Cox  Processes}\label{sec:GP}
Given a test point $\xstar$, inference requires solving the integral $p(\ystar | \xstar, \hyperparam) = \int p( \ystar | \fstar,\xstar) p(\fstar | \dataset, \xstar, \hyperparam) d \fstar$
%\begingroup\makeatletter\def\f@size{8}\check@mathfonts
%\begin{align} \label{eq:predictive_y_distribution}
%p(\ystar | \xstar, \hyperparam) = \int p( \ystar | \fstar,\xstar) p(\fstar | \dataset, \xstar, \hyperparam) d \fstar  \text{,}
%\end{align}
%\endgroup
where $ p(\fstar | \dataset, \xstar, \hyperparam) $ represents the predictive distribution for the test latent function, which in turn is derived as $p(\fstar | \dataset, \xstar, \hyperparam) = \int p(\fstar | \xstar,\f,\hyperparam) p(\f | \dataset,\hyperparam) d \f $ where $p(\f | \dataset,\hyperparam)$ denotes the posterior distribution on the latent functions. Unfortunately, as we are dealing with non-Gaussian likelihoods, this posterior distribution is analytically intractable  and we  we need to resort to approximations to estimate it. \citet{diggle2013spatial} propose a \mala algorithm in which the design of the proposal distribution is a mix of a random walk and a Langevian proposal kernel. As reported by the authors, inference for this class of models is challenging both in terms of computational cost and mixing properties of the \mcmc chain. We will describe our extension of the \lgcp to  multi-task learning problems with our  log Gaussian Cox process network (\lgcpn) model in  \secref{sec:MTCP-model} and the corresponding posterior inference algorithm in \secref{sec:variational-inference}. 
\edwin{Make sure that when we describe what we mean by multi-task, when using it above}

















  

==> mtpp_comparison.tex <==
\section{MTPP comparison}

\begin{table}[t]
	\caption{Coverage of the 90\% CI for the predicted events counts.Values are reported as (In-sample/Out-of-sample).}
	\label{tab:coverage_synthetic_time}
	\begin{center}
		\resizebox{0.49\textwidth}{!}{\begin{tabular}{lccccccccccc}
				\toprule
				\multirow{3}{*}{} &
				\multicolumn{10}{c}{Coverage } \\
				& \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10}\\
				\midrule
				{\lgcpnnormal} & 1.00/1.00  & 1.00/1.00  & 0.95/0.99 & 0.66/1.00  & 1.00/0.86 & 0.97/1.00 & 0.99/1.00  & 0.88/1.00  & 0.92/0.95 & 1.00/1.00 &  \\
				{\mtpp} &  0.77/0.77 &   0.82/0.73  &  0.86/1.00  &  0.93/1.00  &  0.75/0.83  & 0.96/0.84   & 0.78/0.54 &  0.99/1.00 & 0.66/0.88  & 0.74/0.95 \\

				\bottomrule
		\end{tabular}}
	\end{center}
\end{table}

==> performance_fig.tex <==
%\hspace{0.1cm}
%	\begin{minipage}{0.49\textwidth}
%		\vspace{0.5cm}
%		\includegraphics[width=7cm,height=2.5cm]{figs/synthetic/1D/perf_synthetic_2}
%		%[width=0.49\textwidth, valign = c]
%		\vspace{0.1cm}
%		\includegraphics[width=7cm,height=2.5cm]{figs/real/crime_data/nlpl_epochs_crime}
%		\captionof{figure}{\nlpl performance over time. \textit{First row:} synthetic dataset, \textit{Second row:} \crime dataset.}
%		\label{fig:time_perf}
% \end{minipage}
\begin{figure}[t]
	\includegraphics[width=0.3\textwidth]{figs/synthetic/1D/perf_synthetic_2} 
	\includegraphics[width=0.3\textwidth]{figs/real/crime_data/nlpl_epochs_crime}
	\caption{\nlpl performance over time. \textit{First row:} synthetic dataset, \textit{Second row:} \crime dataset.}
	\label{fig:time_perf}
\end{figure}


==> preamble_nips.tex <==
% if you need to pass options to natbib, use, e.g.:
\PassOptionsToPackage{numbers, sort&compress}{natbib}
% before loading nips_2018


% ready for submission
\usepackage{aistats2019}

% to compile a preprint version, e.g., for submission to arXiv, add
% add the [preprint] option:
% \usepackage[preprint]{nips_2018}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2018}

% to avoid loading the natbib package, add option nonatbib:
% \usepackage[nonatbib]{nips_2018}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography


==> related_old.tex <==
\section{Related Work}
%lit review - Diggle/Cressie/Duke/Wilson/AISTATS/NIPS/ICML papers review
%
% MTL IN GENERAL
%
%Multi-Task Log Gaussian Cox Processes (mtLGCPs) as multi-task learning of LGCPs in order to efficiently capture and exploit the potential cross-correlation structure between multiple Log Gaussian Cox processes.
Multi-task learning \citep[\mtl,][]{caruana1998multitask} can improve the generalization ability of multiple learning tasks by sharing common latent representations and transferring information contained in these tasks when they are related. \mtl methods have been developed for a variety of supervised learning algorithms from decision trees \citep{caruana1998multitask}, Gaussian processes \citep[\gptext{s},][]{bonilla2007kernel,bonilla2008multi,titsias2011spike}, to kernel machines and regularization approaches \citep{evgeniou2005learning,argyriou2007multi,argyriou2008convex}; see \citet{zhang2017survey} for a recent survey.  %\theo{Add some more refs like Seager, minka etc?}
% MTL FOR REGRESSION AND  INFERENCE IN GP MODELS WITH NON-LINEAR LIKELIHOODS
A large proportion of the literature on \mtl methods with \gptext{s} has focused on regression problems \citep{bonilla2008multi,teh-et-al-aistats-05,wilson-et-al-icml-12,alvarez2010efficient,alvarez2011computationally}, perhaps due to the additional challenges posed by complex non-linear non-Gaussian likelihood models. However, recent advances in variational inference \cite{2009variational} have allowed the development of more general frameworks with multiple latent functions and multiple outputs \citep{dezfouli2015scalable,hensman-et-al-aistats-2015,gal-et-al-nips-2014}.
%  
%
%A variety of approximation methods, both stochastic such as Markov Chain Monte Carlo algorithms (MCMC; see e.g. \cite{robert2004monte} for a review) and deterministic such as Laplace approximation (see e.g. \cite{mackay2003information}) and expectation propagation (see e.g. \cite{minka2001expectation})
%
% LGCP MODELS
%
%The log-intensity of an LGCP is driven by a single latent Gaussian Process (GP), a stochastic process defined as a collection of random variables, any finite number of which have a multivariate Gaussian distribution \cite{williams2006gaussian}. Typically when the likelihood is non-Gaussian we cannot rely on conjugacy for a closed form posterior over the latent function and have to resort to approximate inference, either stochastic with MCMC sampling schemes \cite{robert2004monte,murray2010elliptical,filippone2014pseudo} or deterministic approximations such as Laplace \cite{mackay2003information}, expectation propagation \cite{minka2001expectation, kuss2005assessing} or variational techniques \cite{girolami2006variational,nguyen2014automated}.

In the specific case of \lgcp models, posterior estimation requires approximate inference methods. Some authors have adopted deterministic approaches such as variational inference \citep{dezfouli2015scalable}, or stochastic approximations based on \mcmc  \citep{diggle2013spatial}. Rather than using a \gptext prior over the log intensity,  other authors consider different non-\lgcp transformations of the latent GPs. Some studies focus on Permanental processes, where a \gptext prior is used over the squared root of the intensities \citep{pmlr-v70-walder17a,lloyd-icml-2015,pmlr-v37-lian15, lloyd2016latent}, others consider a sigmoidal transformation of the latent GPs \citep{adams2009tractable}. Finally, other authors study Convolution processes \citep{gunter2014efficient}).
% MTL LGCP
Our framework can be contrasted with the recently proposed \mlgcp \citep{diggle2013spatial,taylor2015bayesian}, which models the task-specific log-intensity as the sum of a shared \gptext and a task-specific \gptext while performing inference via the Metropolis-adjusted Langevin (\mala). However, this algorithm's performance is hampered by slow mixing in this setting \cite{diggle2013spatial}. Instead we work with a weighted linear combination of  latent base \gptext{s}, where the weights are random, and we offer an efficient variational posterior approximation for this model. 

Finally, our work is related to alternative multivariate formulations such as the linear coregionalization model (\lcm) or the intrinsic coregionalization model (\icm) where the random fields are allowed to covary across the domain via a linear model \citep{alvarez6251kernels}. In the Bayesian treatment of \lcm \citep{schmidt2003bayesian}, the weight parameters have an inverse Wishart prior and inference proceeds with \mcmc. The multivariate \lgcp under \mcmc and even \inla \citep{rue2009approximate} approximations have been prohibitive beyond the simple bivariate setting due to computational cost \citep{shirota2016inference}, identifiability problems and slow convergence \citep{diggle2013spatial} in the case of \mcmc approaches. \lgcpn offers an efficient variational approximation of a Bayesian \lcm that, while being more powerful and robust, also capture uncertainty on the mixing weights.
